Probabilistic proof for non-survival at criticality : the Galton-Watson process and more

In a famous paper, Bezuidenhout and Grimmett demonstrated that the contact process dies out at the critical point.Their proof technique has often been used to study the growth of population patterns. The present text is intended as an introduction to their ideas, with examples of minimal technicality. In particular, we recover the basic theorem about Galton-Watson chains: except in a degenerate case, survival is possible only if the fertility rate exceeds 1. The classical proof that is taught in classrooms is essentially analytic, based on generating functions and convexity arguments. Following the Bezuidenhout-Grimmett way, we propose a proof that is more consistent with probabilistic intuition. We also study the survival problem for a cooperative model, mixing sexual and asexual reproduction.

==> code-julia-3.tex <==
using AbstractAlgebra

function compute_proba(p,q)
 ex=0
 for a=0:1,b=0:1,c=0:1,d=0:1,e=0:1,f=0:1
     s=a+b
     t=c+d+e+f
     z=p^s*(1-p)^(2-s)*q^t*(1-q)^(4-t)
     m=min(s,t)
     ex+=m*z
 end
 return(ex)
end
 
A, (p,q)=polynomial_ring(ZZ,[:p, :q])
chaine="h(p,q)="*repr(compute_proba(p,q))
println(chaine)
eval(Meta.parse(chaine))

# from now on
# h(p,q)=4*p^2*q^4-12*p^2*q^3+12*p^2*q^2-
#   4*p^2*q-2*p*q^4+8*p*q^3-12*p*q^2+8*p*q

using Plots
using Distributed
using Distributions
using DistributedArrays

@everywhere using Distributions

println(workers())

@everywhere function transition(a,b,p,q)
    distA=Binomial(2*(a+b),q)
    distB=Binomial(2*min(a,b),p)
    A=rand(distA,1)[1]
    B=rand(distB,1)[1]
 return(A,B)
end

@everywhere function testedeux(N,survie,p,q=p/2)
    s=0
    for i=1:N
    a=Integer(1)
    b=Integer(1)
    while (a>0) && (b>0) && (b<survie) && (a<survie)
        (a,b)=transition(a,b,p,q)
    end
    s+=(a>0) && (b>0)
end
return(s/N)
end

function q_critique(pp)    
    qmin=0
    qmax=1
    milieu=0.5
    while ((qmax-qmin)>10^(-12))
        milieu=(qmin+qmax)/2
        if (h(pp,milieu)<1)
            qmin=milieu
        else
            qmax=milieu
        end
    end
    return(milieu)
end


pas=0.00125*1
NMC=1000
interv=0:pas:1
survie=@DArray [testedeux(NMC,10^8,i,j)
                   for i=interv,j=interv]
survie_simul=convert(Array,survie)
heatmap(interv,interv,survie_simul,ratio=1,xlabel="q",
ylabel="p",c=reverse(cgrad(:default)),size=(1200,800))

y=0.5:0.01:1
plot!(q_critique.(y),y,linewidth=2,linestyle=:dash,
color=:green,label="h(p,q)=1")
savefig("survival_both_species_with_dot_and_legend.png")
plot!(1/6:0.01:1,q->max(0.5,0.25/q-0.5),linewidth=2,
linestyle=:dash,color=:blue,label="critical")
savefig("Survival_both_species_with_lines.png")
